Arbitrary Virtual Try-On Network: Characteristics Preservation and Trade-off between Body and Clothing

Deep learning based virtual try-on system has achieved some encouraging progress recently, but there still remain several big challenges that need to be solved, such as trying on arbitrary clothes of all types, trying on the clothes from one category to another and generating image-realistic results with few artifacts. To handle this issue, we in this paper first collect a new dataset with all types of clothes, \ie tops, bottoms, and whole clothes, each one has multiple categories with rich information of clothing characteristics such as patterns, logos, and other details. Based on this dataset, we then propose the Arbitrary Virtual Try-On Network (AVTON) that is utilized for all-type clothes, which can synthesize realistic try-on images by preserving and trading off characteristics of the target clothes and the reference person. Our approach includes three modules: 1) Limbs Prediction Module, which is utilized for predicting the human body parts by preserving the characteristics of the reference person. This is especially good for handling cross-category try-on task (\eg long sleeves \(\leftrightarrow\) short sleeves or long pants \(\leftrightarrow\) skirts, \etc), where the exposed arms or legs with the skin colors and details can be reasonably predicted; 2) Improved Geometric Matching Module, which is designed to warp clothes according to the geometry of the target person. We improve the TPS based warping method with a compactly supported radial function (Wendland's \(\Psi\)-function); 3) Trade-Off Fusion Module, which is to trade off the characteristics of the warped clothes and the reference person. This module is to make the generated try-on images look more natural and realistic based on a fine-tune symmetry of the network structure. Extensive simulations are conducted and our approach can achieve better performance compared with the state-of-the-art virtual try-on methods.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> abstract_bak.tex <==
% \begin{abstract}
% Image-based virtual try-on system has been paid considerable attention recently. Although some encouraging progress has been made, developing a realistic and arbitrary virtual try-on method is less successful and still requires further research. Hence, we propose the Improved Characteristic-Preserving Arbitrary Virtual Try-On Network (ICPA-VTON) that is suitable for arbitrary styles of clothes, and it can synthesize realistic try-on images to preserve more characteristics of the target clothes and the reference person than priors. Our approach includes three modules. First, the Limbs Prediction Module (LPM) aims at predicting the limbs of the reference person roughly, it is useful in the task of generating reasonable lengths of exposed limbs (when long sleeves\(\leftrightarrow\)short sleeves or long pants\(\leftrightarrow\)skirts, etc.), and can outline the general shape and posture of the human body for the next modules to preserve more characteristics of the reference person. Second, the Improved Geometric Matching Module (IGMM) uses radial basis function (Wendland's \(\Psi\)-function) with compact support for elastic registration of warping clothes, it allows to constrain elastic deformations to image parts required and preserve more characteristics of the target clothes. Third, the Improved Try-On Module (ITOM) can deal with arbitrary styles of clothes and trade off characteristics of the target clothes and the reference person due to two pairs of UNets. It extracts features from the target clothes and the reference person respectively, and then fuses them together to get the realistic try-on image. In comparison to the state-of-the-art methods, our approach fits in better with arbitrary virtual try-on tasks and provides more realistic images qualitatively and quantitatively.
% \end{abstract}
\begin{abstract}
Image-based virtual try-on system has been paid considerable attention recently. Although some encouraging progress has been made, developing an arbitrary and realistic virtual try-on method is less successful and still requires further research. A case in point is that most current virtual try-on methods are developed based on VITON dataset that only contains frontal-view and top clothing image pairs, so that the arbitrary virtual try-on for the whole categories of clothes cannot be realized (Fig. \ref{fig: beginning}). To handle this issue, we in this paper propose an Improved Characteristic-Preserving Arbitrary Virtual Try-On Network (ICPA-VTON) that is utilized for arbitrary styles of clothes, which can synthesize realistic try-on images by preserving more characteristics of the target clothes and the reference person. Our approach includes three modules. First, the Limbs Prediction Module (LPM) aims at predicting the limbs of the reference person, which is effective in the task of generating reasonable and realistic exposed limbs (when long sleeves\(\leftrightarrow\)short sleeves or long pants\(\leftrightarrow\)skirts, etc.). As a result, the general shape and posture of the human body with the predicted limbs can be transferred to the next modules to preserve more characteristics of the reference person; second, to character the clothes image when warping it an arbitrary human pose, an Improved Geometric Matching Module (IGMM) is proposed for elastic registration of warping clothes. By adopting the radial basis function (Wendland's \(\Psi\)-function), it allows to constrain elastic deformations to image parts and preserve more characteristics of the target clothes; third, the Improved Try-On Module (ITOM) is developed, which can deal with arbitrary styles of clothes and trade off characteristics of the target clothes and the reference person due to two pairs of UNets. In detail, it firstly extracts the features from the target clothes and the reference person respectively, and then fuses them together to get the realistic try-on image. Extensive simulations are conducted and compared with the state-of-the-art virtual try-on methods, our approach can achieve better performance in arbitrary virtual try-on tasks and provide more realistic images both in qualitatively and quantitatively.
\end{abstract}

==> introduction_bak.tex <==
% \section{Introduction}
% In recent years, with the increasing demands of online shopping for fashion items, item suitability has influential impact to online shopping, because consumers tend to consider whether it fit when finalizing purchase decisions. In order to meet the shopping needs of consumers, researchers have conducted considerable researches on image-based virtual try-on technology. Although these researches has made some progress, it remains some ongoing challenges to produce realistic try-on results and adapt try-on system to any task. Current works focus on top clothing try-on task due to the lack of diversity in the dataset, and the result generated is not realistic enough due to the shortcomings of the method.

% Specifically, the dataset used in most prior arts is VITON dataset that only contains frontal-view woman and top clothing image pairs. Although theoretically a model that can perform better on top clothing try-on task can also perform the same on the other tasks through retraining, it is still difficult to adapt one trained model to various tasks.
% Therefore, we need a dataset containing tops, bottoms and wholes. To increase the diversity of the dataset, we collected a new dataset from the \href{https://www.zalando.co.uk}{Zalando}. As shown in Fig. \ref{fig: beginning}, the example in the first row represents top clothing try-on task, this type of data is similar to VITON dataset, but it is richer in characteristics. Such as human images of all genders, these images include various shapes and poses, and top clothing images with rich patterns, various styles and so on. As can be seen From the example on the second row, the human images for bottom clothing try-on task are generally lower limbs, and the bottom clothing images include trousers, shorts and  skirts, etc., and have rich textures, logos and other details. The last row presents examples for whole clothing try-on task, where this type of human images generally contains the entire human body, and most of the whole clothing images are dresses.
\section{Introduction}
In modern society, clothing plays an important role in human daily life, as proper outfit can enhance peoples’ beauty and personal quality. But in practice, people tend to make final purchase decision before trying on the clothes. On the other hand, huge amounts of clothing data emerge in the Internet or social media during the past few years due to the development of the clothing e-commerce platform. It is impossible and unfeasible try on all the clothes especially in the web. Therefore, to meet the shopping needs of consumers, it is necessary for researchers to conducted considerable researches on image-based virtual try-on technology \cite{hauswiesner2013virtual, iccv2017fashiongan}, where the goal is to achieve a photo-realistic try-on effects on website or smartphone app by transforming the target clothing outfit onto a certain reference person.

During the past few years, computer vision technology has been widely utilized in the extensive applications of artificial fashion. These applications typically include clothes detection \cite{ liuLQWTcvpr16DeepFashion, DeepFashion2}, clothes parsing \cite{li2019self, liang2015deep, li2017multiple, gong2017look}, clothes attributions and categories recognition \cite{ wang2018toward, liuLQWTcvpr16DeepFashion, DeepFashion2}, clothes collocation \cite{ iwata2011fashion, zhao2020end, veit2015learning, he2016learning, shih2018compatibility, li2017mining, han2017learning, cui2019dressing}, clothes image retrieval \cite{ zeng2020tilegan, liu2018deep, liuYLWTeccv16FashionLandmark, guo2019fashion, lin2020fashion, hosseinzadeh2020composed, jandial2020trace} and fashion edit \cite{hsiao2019fashion++,dong2019fashion}. These applications are all merited from recently
developed technology, namely deep learning due to its powerful feature extraction ability to capture the rich mid-level image representations. Motivated by this technology, the deep learning based virtual try-on methods has been extensively studied and achieved considerable results. These methods have adopted the concept of GAN and focus on generalizing the synthetical and photo-realistic try-on images by preserving the characteristics of a clothing image (e.g., texture, logo, and embroidery) as well as warping it to an arbitrary human pose. Typical method include VITON \cite{han2018viton}, CP-VTON \cite{wang2018toward}, VTNFP \cite{yu2019vtnfp}, ACGPN \cite{yang2020towards}, et al. \cite{pandey2020poly, neuberger2020image, raj2018swapnet,pons2017clothcap, mo2018instagan, guan2012drape, iccv2017fashiongan, han2019compatible}. Although these researches has made some progress, it remains some ongoing challenges to produce realistic try-on results.

On the one hand, current works mainly focus on top clothing try-on task due to the lack of diversity in the dataset. Specifically, the dataset used in most prior arts is VITON dataset that only contains frontal-view woman and top clothing image pairs. Although theoretically a model that can perform better on top clothing try-on task can also perform the same on the other tasks through retraining, it is still difficult to adapt one trained model to various tasks.
Therefore, we need a dataset containing tops, bottoms and wholes. 

To increase the diversity of the dataset, we collected a new dataset from the \href{https://www.zalando.co.uk}{Zalando}. As shown in Fig. \ref{fig: beginning}, the example in the first row represents top clothing try-on task, this type of data is similar to VITON dataset, but it is richer in characteristics. Such as human images of all genders, these images include various shapes and poses, and top clothing images with rich patterns, various styles and so on. As can be seen from the example on the second row, the human images for bottom clothing try-on task are generally lower limbs, and the bottom clothing images include trousers, shorts and  skirts, etc., and have rich textures, logos and other details. The last row presents examples for whole clothing try-on task, where this type of human images generally contains the entire human body, and most of the whole clothing images are dresses.

On the other hand, the result generated is not realistic enough due to the shortcomings of the prior methods. Firstly, some methods cannot preserve the characteristics of the target clothes, such as VITON. The main reason for its failure is the coarse-to-fine strategy and the imperfect matching module, which result in blurry clothes. Secondly, some methods cannot preserve the characteristics of the reference person, such as CP-VTON, Poly-GAN and VTNFP. Among these examples, CP-VTON has problems with limb being covered by clothes; Poly-GAN is failure to generate reasonable color of skin; and VTNFP cannot generate detailed hands. Thirdly, the other prior methods are not good at trading off characteristics of the 
warped clothes and the reference person, such as ACGPN. Although it can preserve the characteristics of the warped clothes and reference person as much as possible, its generated images is not realistic enough, such as some artifacts near the neck regions. The reason for this result is that the final fusion module tends to preserve warped clothing characteristics and cannot correct these errors. 

To address the issues mentioned above, we propose a new image-based virtual try-on method, called ICPA-VTON. It contains three modules: 1) Limbs Prediction Module for predicting limbs and preserving head and non-target parts, it aims at preserving the characteristics of the reference person; 2) Improved Geometric Matching Module is designed to warped clothes precisely. Different from CP-VTON, we replace TPS with Wendland's \(\Psi\)-function, which warps clothes locally, limits deformation and preserves the characteristics of the target clothes; 3) Improved Try-On Module, which can trade off the characteristics of the warped clothes and the reference person, the generated try-on images looks natural and real due to the symmetry of the network structure (a pair of UNet). Experiments show that ICPA-VTON significiantly improved the state-of-the-art methods for virtual try-on method, and can generate realistic try-on images in the arbitrary virtual try-on task (Fig. \ref{fig: beginning}).

The main contributions of this paper are summarized as follows:
\begin{enumerate}
    \item We collected a new dataset that is more diverse. It contains the whole categories of clothes. Benefiting from this dataset, we designed a method that adapts to arbitrary virtual try-on task.
    \item We propose a new limbs prediction module to predict limbs and preserve the characteristics of the reference person. We show that it is necessary in complex try-on tasks.
    \item We for the first time use the \(\Psi\)-function of Wendland to warp clothes that is compact support for the registration of images. It greatly improves the try-on quality in preserving the characteristics of the target clothes.
    \item We present a novel fusion network that trades off the characteristics of the warped clothes and the reference person. By adjusting characteristics and correcting errors, the try-on images are more realistic.
    \item We demonstrate that our proposed method can be applied to arbitrary virtual try-on task, and outperforms the state-of-the-art methods both qualitatively and quantitatively.
\end{enumerate}
